Federated Cross-Modal Retrieval with Missing Modalities via Semantic Routing and Adapter Personalization

Federated cross-modal retrieval faces severe challenges from heterogeneous client data, particularly non-IID semantic distributions and missing modalities. Under such heterogeneity, a single global model is often insufficient to capture both shared cross-modal knowledge and client-specific characteristics. We propose RCSR, a personalization-friendly federated framework that integrates prototype anchoring, retrieval-centric semantic routing, and optional client-specific adapters. Built on a frozen CLIP backbone, RCSR leverages lightweight shared adapters for global knowledge transfer while supporting efficient local personalization. Prototype anchoring helps unimodal clients align with global cross-modal semantics, and a server-side semantic router adaptively assigns aggregation weights based on retrieval consistency to mitigate alignment drift during heterogeneous updates. Extensive experiments on MS-COCO, Flickr30K, and other benchmarks show that RCSR consistently improves global retrieval accuracy and training stability, while further enhancing client-level retrieval performance, especially for clients with incomplete modalities. Code is available at https://github.com/RezinChow/RCSR-Retrieval-Centric-Semantic-Routing.

==> CA.tex <==
\subsection{Client-Specific Adapter Personalization}
\label{sec:personalization}

While RCSR improves average retrieval quality across heterogeneous clients, a single shared model may not optimally serve all participants given their diverse data distributions and modality availability. We introduce per-client personalization adapters whose adaptation intensity is guided by the router's aggregation weights, yielding \textbf{RCSR-p}.

\textbf{Adapter Architecture.}
Each client $k$ maintains a lightweight personalization adapter $A_k\colon \R^d \to \R^d$ applied as a residual correction to the shared encoder output:
\begin{equation}\label{eq:personalized}
\tilde{z}_k = z + s_k \cdot A_k(z), \quad A_k(z) = W_2\,\mathrm{GELU}(W_1 z),
\end{equation}
where $W_2$ is initialized to near-zero so that $A_k$ begins as an approximate identity, ensuring minimal disruption to the global representation at personalization onset. The adapter is applied independently to image and text embeddings.

\textbf{Router-Guided Personalization Strength.}
The scalar $s_k \in (0, 0.5]$ ties adaptation intensity to the router weight $w_k^R$, which quantifies client $k$'s contribution to global retrieval coherence. Clients the router down-weights---due to alignment drift, limited paired data, or conflicting alignment directions---benefit more from local adaptation:
\begin{equation}\label{eq:strength}
s_k = \min\!\bigl(\lambda_p \cdot (1 + \max(0,\;0.5 - w_k^R)),\;0.5\bigr),
\end{equation}
where $\lambda_p$ is a base strength hyperparameter. This inverse coupling ensures that clients whose updates are already trusted globally receive only mild local correction, while clients underserved by the global model receive proportionally stronger compensation. Crucially, this signal is derived from existing router computation with no additional communication.

\textbf{Personalization Training.}
Personalization begins at round $T_p$ once the global model has stabilized. After each standard local training step, client $k$ performs additional adapter fine-tuning at a reduced learning rate $(0.1\eta)$. Paired clients minimize $\mathcal{L}_{\mathrm{NCE}}$ (Eq.~\ref{eq:infonce}) computed on personalized features $\tilde{z}_{k,I},\tilde{z}_{k,T}$; single-modality clients anchor their personalized features to the complementary global prototype via $\mathcal{L}_{\mathrm{anchor}}$ (Eq.~\ref{eq:anchor}). Adapter parameters $\{A_k\}$ are \emph{never} aggregated to the server---only the global shared adapters and projection heads participate in federated aggregation---keeping per-client personalization entirely local and communication-free.


==> discussion.tex <==
\subsection{Discussion}

\textbf{Fairness and average performance are aligned.} The minimax game raises the worst-case client's absolute performance (0.45 vs.\ 0.43 for FedAvg at MR=50\%) rather than merely redistributing scores---an outcome we attribute to the geometric structure of retrieval tasks, where undertrained clients inject alignment noise that degrades the shared embedding space for all clients.

\textbf{When does personalization help most?} RCSR-P's gains over RCSR are largest for clients with low router weight (typically single-modality or highly non-IID clients). For these clients, the router already signals that their updates conflict with the global objective; stronger local adaptation (Eq.~\ref{eq:strength}) compensates by specializing the encoder output to their local distribution without affecting the globally aggregated parameters.

\textbf{Computational overhead.} The router's forward pass processes $K=10$ client statistics through 2 transformer layers ($<$50ms on a V100 GPU), negligible relative to local training ($\sim$2 min/round/client). Communication cost increases by only $\sim$1\% (statistics are $\sim$10KB per client vs.\ $\sim$12MB for model parameters). Per-client adapters add no communication cost as they remain entirely local.



==> his_tabel.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison on Flickr30K under different missing modality rates. All methods trained with 30 clients for 150 rounds ($\alpha=0.1$). Best results in \textbf{bold}.}
\label{tab:flickr30k_missing_rate}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|ccc|ccc|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{MR}} & \multicolumn{3}{c|}{\textbf{Image-to-Text}} & \multicolumn{3}{c|}{\textbf{Text-to-Image}} & \multirow{2}{*}{\textbf{$\bar{R}$@1}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
& & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & \\
\midrule
FedAvg      & 0\%  & 45.49 & 73.99 & 82.89 & 44.86 & 73.95 & 82.89 & 45.17 \\
RCSR (Ours) & 0\%  & \textbf{45.49} & \textbf{74.21} & \textbf{83.52} & \textbf{45.71} & \textbf{74.83} & \textbf{83.27} & \textbf{45.27} \\
\midrule
FedAvg      & 30\% & 39.86 & 70.84 & 80.69 & 41.24 & 70.62 & 81.47 & 40.55 \\
RCSR (Ours) & 30\% & \textbf{42.15} & \textbf{71.82} & \textbf{81.63} & \textbf{43.88} & \textbf{72.26} & \textbf{81.94} & \textbf{43.02} \\
\midrule
FedAvg      & 50\% & 36.46 & 67.51 & 77.51 & 38.57 & 68.07 & 77.82 & 37.51 \\
FedProx     & 50\% & 37.92 & 68.74 & 78.65 & 39.84 & 69.23 & 79.01 & 38.88 \\
CreamFL     & 50\% & 40.23 & 70.58 & 80.12 & 41.65 & 71.02 & 80.46 & 40.94 \\
RCSR (Ours) & 50\% & \textbf{46.78} & \textbf{75.59} & \textbf{84.11} & \textbf{47.94} & \textbf{74.83} & \textbf{83.74} & \textbf{47.36} \\
\midrule
FedAvg      & 70\% & 29.29 & 58.26 & 70.18 & 29.51 & 58.16 & 71.03 & 29.40 \\
RCSR (Ours) & 70\% & \textbf{36.85} & \textbf{64.42} & \textbf{75.70} & \textbf{38.25} & \textbf{66.62} & \textbf{78.06} & \textbf{37.55} \\
\bottomrule
\end{tabular}%
}
\end{table}


\begin{table}[t]
\centering
\caption{Ablation study on Flickr30K with 50\% missing modality rate. All variants trained with 30 clients for 150 rounds ($\alpha=0.1$). Best results in \textbf{bold}.}
\label{tab:flickr30k_ablation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|ccc|c}
\toprule
\multirow{2}{*}{\textbf{Method Variant}} & \multicolumn{3}{c|}{\textbf{Image-to-Text}} & \multicolumn{3}{c|}{\textbf{Text-to-Image}} & \multirow{2}{*}{\textbf{$\bar{R}$@1}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & \\
\midrule
RCSR Full (Ours)          & \textbf{46.78} & \textbf{75.59} & \textbf{83.99} & \textbf{47.94} & \textbf{74.83} & \textbf{83.74} & \textbf{47.36} \\
\quad w/o Minimax Game    & 37.53          & 67.16          & 78.86          & 39.67          & 68.39          & 79.08          & 38.60 \\
\quad w/o Client Align    & 39.51          & 69.30          & 80.65          & 41.08          & 70.65          & 80.87          & 40.30 \\
\midrule
\textit{Drop w/o Minimax}      & \textcolor{red}{-9.25} & \textcolor{red}{-8.43} & \textcolor{red}{-5.13} & \textcolor{red}{-8.27} & \textcolor{red}{-6.44} & \textcolor{red}{-4.66} & \textcolor{red}{-8.76} \\
\textit{Drop w/o Client Align} & \textcolor{red}{-7.27} & \textcolor{red}{-6.29} & \textcolor{red}{-3.34} & \textcolor{red}{-6.86} & \textcolor{red}{-4.18} & \textcolor{red}{-2.87} & \textcolor{red}{-7.06} \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[t]
\centering
\caption{Sensitivity to data heterogeneity on Flickr30K (30 clients, MR=50\%). Lower $\alpha$ indicates more severe non-IID. Best results in \textbf{bold}.}
\label{tab:alpha_sensitivity}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|l|ccc|ccc|c|c}
\toprule
\multirow{2}{*}{\textbf{$\alpha$}} & \multirow{2}{*}{\textbf{Heterogeneity}} & \multicolumn{3}{c|}{\textbf{Image-to-Text}} & \multicolumn{3}{c|}{\textbf{Text-to-Image}} & \multirow{2}{*}{\textbf{$\bar{R}$@1}} & \multirow{2}{*}{\textbf{Fair. Std}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
& & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & & \\
\midrule
0.01  & Extreme   & 39.51 & 67.29 & 76.85 & 39.67 & 68.61 & 78.46 & 39.59 & 0.0980 \\
0.10  & Severe    & \textbf{46.78} & \textbf{75.59} & \textbf{84.11} & \textbf{47.94} & \textbf{74.83} & \textbf{83.74} & \textbf{47.36} & \textbf{0.0382} \\
10.0  & Mild (IID) & 39.04 & 69.36 & 79.31 & 39.67 & 69.74 & 79.93 & 39.35 & 0.0267 \\
\bottomrule
\end{tabular}%
}
\end{table}


\begin{table}[t]
\centering
\caption{Client scaling analysis on Flickr30K with $\alpha=0.1$, MR=50\%. Best results in \textbf{bold}.}
\label{tab:client_scaling}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc|c|c}
\toprule
\multirow{2}{*}{\textbf{\#Clients}} & \multicolumn{3}{c|}{\textbf{Image-to-Text}} & \multicolumn{3}{c|}{\textbf{Text-to-Image}} & \multirow{2}{*}{\textbf{$\bar{R}$@1}} & \multirow{2}{*}{\textbf{Fair. Std}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & & \\
\midrule
5  & \textbf{49.32} & \textbf{77.60} & \textbf{85.58} & \textbf{50.17} & \textbf{76.79} & \textbf{85.25} & \textbf{49.75} & 0.0753 \\
15 & 43.72 & 74.14 & 83.25 & 45.14 & 74.02 & 83.06 & 44.43 & 0.0494 \\
30 & 46.78 & 75.59 & 84.11 & 47.94 & 74.83 & 83.74 & 47.36 & \textbf{0.0382} \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[t]
\centering
\caption{Performance comparison on MS-COCO under different missing modality rates. All methods trained with 30 clients for 150 rounds ($\alpha=0.1$). Best results in \textbf{bold}.}
\label{tab:coco_missing_rate}
\resizebox{\columnwidth}{!}{%
FedAvg      & 0\%  & 40.84 & 69.00 & 80.06 & 41.08 & 68.60 & 79.68 & 40.96 \\
RCSR (Ours) & 0\%  & \textbf{41.52} & \textbf{70.72} & \textbf{81.08} & \textbf{41.98} & \textbf{71.16} & \textbf{81.12} & \textbf{41.75} \\
\midrule
FedAvg      & 30\% & 37.08 & 66.66 & 78.48 & 39.78 & 66.98 & 78.16 & 38.43 \\
RCSR (Ours) & 30\% & \textbf{39.40} & \textbf{67.28} & \textbf{79.02} & \textbf{40.68} & \textbf{68.04} & \textbf{78.40} & \textbf{40.04} \\
\midrule
FedAvg      & 50\% & 35.26 & 63.68 & 76.06 & 36.14 & 63.84 & 75.58 & 35.70 \\
FedProx     & 50\% & 36.18 & 64.52 & 76.78 & 37.22 & 64.96 & 76.34 & 36.70 \\
CreamFL     & 50\% & 37.42 & 65.86 & 77.24 & 38.58 & 66.18 & 77.02 & 38.00 \\
RCSR (Ours) & 50\% & \textbf{38.26} & \textbf{66.24} & \textbf{77.88} & \textbf{39.46} & \textbf{66.92} & \textbf{77.40} & \textbf{38.86} \\
\midrule
FedAvg      & 70\% & 29.06 & 56.00 & 69.68 & 30.26 & 57.48 & 70.30 & 29.66 \\
RCSR (Ours) & 70\% & \textbf{35.68} & \textbf{63.82} & \textbf{74.96} & \textbf{37.34} & \textbf{65.06} & \textbf{76.22} & \textbf{36.51} \\
\bottomrule
\end{tabular}%
}
\end{table}
